MetaCoCo: A New Few-Shot Classification Benchmark with Spurious Correlation

Out-of-distribution (OOD) problems in few-shot classification (FSC) occur when novel classes sampled from testing distributions differ from base classes drawn from training distributions, which considerably degrades the performance of deep learning models deployed in real-world applications. Recent studies suggest that the OOD problems in FSC mainly including: (a) cross-domain few-shot classification (CD-FSC) and (b) spurious-correlation few-shot classification (SC-FSC). Specifically, CD-FSC occurs when a classifier learns transferring knowledge from base classes drawn from seen training distributions but recognizes novel classes sampled from unseen testing distributions. In contrast, SC-FSC arises when a classifier relies on non-causal features (or contexts) that happen to be correlated with the labels (or concepts) in base classes but such relationships no longer hold during the model deployment. Despite CD-FSC has been extensively studied, SC-FSC remains understudied due to lack of the corresponding evaluation benchmarks. To this end, we present Meta Concept Context (MetaCoCo), a benchmark with spurious-correlation shifts collected from real-world scenarios. Moreover, to quantify the extent of spurious-correlation shifts of the presented MetaCoCo, we further propose a metric by using CLIP as a pre-trained vision-language model. Extensive experiments on the proposed benchmark are performed to evaluate the state-of-the-art methods in FSC, cross-domain shifts, and self-supervised learning. The experimental results show that the performance of the existing methods degrades significantly in the presence of spurious-correlation shifts. We open-source all codes of our benchmark and hope that the proposed MetaCoCo can facilitate future research on spurious-correlation shifts problems in FSC. The code is available at: https://github.com/remiMZ/MetaCoCo-ICLR24.

==> section/8_rebuttal.tex <==
\section{Rebuttal}
\textcolor{blue}{\textbf{Review F7NA.}}

We thank all reviewers for their time and thought-provoking feedback! We are excited to see that all reviewers agree that our overall motivation is interesting and novel with the high-quality writing, comprehensive experiments and strong results (\textbf{R\#F7nA},\textbf{R\#QLBK},\textbf{R\#xD6Q}). We address the major concerns in each review.

\textcolor{blue}{\textbf{Review F7NA.}}

\textbf{The performance of vision-language pre-trained models on the MetaCoCo.}
We evaluate the performance of vision-language pre-trained models (VLMs) on our proposed MetaCoCo dataset. These VLMs methods main are divided into zero-shot CLIP and prompt-tuning CLIP. Following their original paper, two representative backbones with 1-shot and 16-shot samples are used, \textit{i.e.}. ResNet50 and ViT-B/16. These experimental resutls are shown as below:
\begin{table}[htbp]  
    \centering
    \caption{Experiments in few-shot classification by using vision-language pre-trained models. Two vision backbones following their original paper are considered, \textit{i.e.}, ResNet50 and ViT-B/16.}
    \vspace{-3mm}
    % \scalebox{0.86}{
    \resizebox{1.0\textwidth}{!}{
        \begin{tabular}{lccc|ccc|ccc}
            \shline
            & & & & \multicolumn{3}{c|}{$1$-shot} & \multicolumn{3}{c}{$16$-shot} \\
            Method & Conference & Backbone & Type & Base & New & HM 
            & Base & New & HM \\
            \hline
            CLIP~[1] & ICML2021 & ResNet50 & Zero-shot CLIP & 68.12 & 72.19 & 70.10 & 68.12 & 72.19 & 70.10   \\
            CoOp~[2] & IJCV2022 & ResNet50 & Prompt-tuning CLIP & 61.22 & 63.62 & 62.40 & 47.55 & 40.90 & 43.98  \\ 
            CoCoOp~[3] & CVPR2022 & ResNet50 & Prompt-tuning CLIP & 59.86 & 63.88 & 61.80 & 36.88 & 46.10 & 40.98 \\
            KgCoOp~[4] & CVPR2023 & ResNet50 & Prompt-tuning CLIP & 67.95 & 72.05 & 69.94 & 49.18 & 48.78 & 48.98 \\
            LFA~[6] & ICCV2023 & ResNet50 & Prompt-tuning CLIP & 66.87 & 73.01 & 69.81 & 49.23 & 48.12 & 48.67 \\
            ProGrad~[7] & ICCV2023 & ResNet50 & Prompt-tuning CLIP & 65.23 & 69.39 & 67.25 & 49.14 & 47.36 & 48.23 \\
            \hline \hline
            CLIP~[1] & ICML2021 & ViT-B/16 & Zero-shot CLIP & 73.19 & 75.29 & 74.23 & 73.19 & 75.29 & 74.23  \\
            CoOp~[2] & IJCV2022 & ViT-B/16 & Prompt-tuning CLIP & 64.95 & 68.87 & 66.85 &  49.98 & 45.40 & 47.58  \\ 
            CoCoOp~[3] & CVPR2022 & ViT-B/16 & Prompt-tuning CLIP & 65.60 & 69.50 & 67.49 & 49.35 & 47.84 & 48.58 \\
            KgCoOp~[4] & CVPR2023 & ViT-B/16 & Prompt-tuning CLIP & 71.22 & 74.74 & 72.94 & 51.21 & 50.99 & 51.10 \\
            MaPLe~[5] & CVPR2023 & ViT-B/16 & Prompt-tuning CLIP & 60.31 & 68.94 & 64.34 & 48.04 & 49.47 &  48.74 \\
            LFA~[6] & ICCV2023 & ViT-B/16 & Prompt-tuning CLIP & 71.56 & 74.98 & 73.23 & 52.04 & 49.65 & 50.82 \\
            ProGrad~[7] & ICCV2023 & ViT-B/16 & Prompt-tuning CLIP & 70.81 & 73.27 & 72.02 & 51.48 & 48.02 & 49.69 \\
            \shline
    \end{tabular}
} 
\label{tab:fsc_acc}
\end{table}

From the table, we can find two interesting but opposite conclusions that (1) The more samples are used in the model prompt-tuning phase, the worse the performance of the model will be. For example, the performance drops from 62.40 with 1-shot to 43.98 with 16-shot in CoOp with ResNet50. This further indicates that the more samples used, the greater the bias in spurious correlations introduced, resulting in reduced model performance. (2) The performance of prompt-tuning methods is lower than zero-shot CLIP in all settings. The possible reason is that prompt-tuning methods overfits to spurious information, therefore, affecting the generalization of the model. 

\textbf{Reference}

[1] Radford Alec et al. Learning transferable visual models from natural language supervision. ICML2021.

[2] Kaiyang Zhou et al. Learning to prompt for vision-language models. IJCV2022.

[3] Kaiyang Zhou et al. Conditional prompt learning for vision-language models. CVPR2022.

[4] Haotao Yao et al. Visual-Language Prompt Tuning with Knowledge-guided Context Optimization. CVPR2023.

[5] Muhammad Uzair Khattak et al. MaPLe: Multi-modal Prompt Learning. CVPR2023.

[6] Yassine Ouali et al. Black Box Few-Shot Adaptation for Vision-Language models. ICCV2023.

[7] Beier Zhu et al. Prompt-aligned Gradient for Prompt Tuning. ICCV2023.

\textcolor{blue}{\textbf{Review QLBK.}}

\textbf{Technical contribution.}

In this paper, 

\textbf{The difference between spurious-correlation studied in this paper and overfitting in few shot learning.}

\textbf{Can we view spurious-correlation as one type of model overfitting?}

\textbf{}

\begin{table}[htbp]  
    \centering
    \caption{Experimental results in few-shot classification methods and these methods aim to solve the overfitting phenomena of the few-shot learning.}
    \vspace{-3mm}
    % \scalebox{0.86}{
    \resizebox{1.0\textwidth}{!}{
        \begin{tabular}{lcccccc|cc}
            \shline
            Method & Conference & Backbone & Type & GL & LL & TT & $1$-shot & $5$-shot \\ 
            \hline
            MTL~[1] & CVPR2019 & ResNet12 & Meta & \cmark & \cmark & \cmark & 44.23 & 58.04 \\
            ProtoNet~[2]  &  NeurIPS2017 & ResNet12 & Metric & & \cmark & \cmark & 42.69 & 59.50 \\
            BF3S~[3] & ICCV2019 & WRN-28-10 & Metric &  & \cmark & \cmark & 43.78  & 57.64 \\
            FEAT~[4] & CVPR2020 & ResNet18 & Metric & \cmark & \cmark & \cmark & 50.23 & 64.12 \\ 
            DSN~[5] & CVPR2020 & ResNet12 & Metric & & \cmark & \cmark & 46.21 & 58.01 \\
            SVM with DC~[6] & TPAMI2021 & ResNet18 & Metric & \cmark & \cmark & \cmark & 43.56 & 58.96 \\
            SMKD with Prototype~[7] & CVPR2023 & ViT-S & Metric  & \cmark & \cmark & \cmark & 56.89 & 69.54 \\
            FGFL~[8] & ICCV2023 & ResNet12 & Metric &  & \cmark & \cmark & 46.78 & 64.32 \\
            LP-FT-FB~[9] & ICLR2023 & ResNet12 & Fine-tuning & \cmark & \cmark & \cmark & 56.21 &  70.21   \\
            \shline
    \end{tabular}
} 
\label{tab:fsc_acc}
\vspace{-4mm}
\end{table}


\textbf{Reference}

[1] Qianru Sun et al. Meta-transfer learning for few-shot learning. CVPR2019. 

[2] Jake Snell et al. Prototypical Networks for Few-shot Learning. NeurIPS2017. 

[3] Spyros Gidaris et al. Boosting Few-Shot Visual Learning With Self-Supervision. ICCV2019. 

[4] Hanjia Ye et al. Few-Shot Learning via Embedding Adaptation with Set-to-Set Functions. CVPR2020. 

[5] Christian Simon et al. Adaptive Subspaces for Few-Shot Learning. CVPR2020. 

[6] Shuo Yang et al. Bridging the Gap Between Few-Shot and
Many-Shot Learning via Distribution Calibration. TPAMI2021. 

[7] Han Lin et al. Supervised Masked Knowledge Distillation  for Few-Shot Transformers. CVPR2023.

[8] Hao Cheng et al. Frequency Guidance Matters in Few-Shot Learning. ICCV2023.

[9] Heng Wang et al. Revisit Finetuning strategy for Few-Shot Learning to Transfer the Emdeddings. ICLR2023. (LP-FT-FB-fine-12)



\textcolor{blue}{\textbf{Review xD6Q.}}

\textbf{Contributions are not clearly and accurately stated.}

In this paper, our main contributions are: (1) we first analyze the importance of studying spurious-correlation shifts in the field of few-shot classification. (2) We present meta concept context (MetaCoCo) dataset, which is a large-scale benchmark with spurious-correlation shifts arising from various contexts in real-world applications. (3) We propose a metric by using CLIP as a pre-trained vision-language model to quantify and compare the extent of spurious correlations on the MetaCoCo and other FSC benchmarks. 

\textbf{The explanation for the spurious-correlation few-shot classification is not easy to understand.}

Few-shot classification (FSC) aims to recognize unlabeled images (or query set) from novel classes with only few labeled images (or support set) by transferring knowledge learned from base classes. If the pre-trained FSC model is tested on the query is dissimilar to that of the support set, the performance of the model is severely compromised. For example, the support set is the dog in the grass but the query set is the dog in the autumn. Therefore, studying spurious-correlation shifts in few-shot classification is interesting and consistent with real-world scenarios.

\textbf{More experiments about recent methods on the proposed MetaCoCo dataset.}

We present more experimental results below to analyze the performance of these recent methods on our proposed MetaCoCo dataset. In addition to these methods mentioned by the reviewer, we also verify the recent state-of-the-art methods including some vision-language pre-trained methods to analyze the performance on our proposed MetaCoCo.

In addition, as suggested by the reviewer, we also compare with the most recent methods, which can be broadly classified into the following 4 types: 

+analysis

\begin{table}[htbp]  
    \centering
    \caption{Experimental results in recent state-of-the-art few-shot classification methods.}
    \vspace{-3mm}
    % \scalebox{0.86}{
    \resizebox{1.0\textwidth}{!}{
        \begin{tabular}{lcccccc|cc}
            \shline
            Method & Conference & Backbone & Type & GL & LL & TT & $1$-shot & $5$-shot \\ 
            \hline
            CDKT+ML~[1] & NeurIPS2023 & ResNet18 & Meta & & \cmark & \cmark & 44.86 & 61.42 \\
            CDKT+PL~[1]  & NeurIPS2023 & ResNet18 & Meta & & \cmark & \cmark & 43.21 & 59.87 \\
            DeepBDC~[2] & CVPR2022 & ResNet12 & Metric & & \cmark & \cmark & 46.78 & 62.54 \\
            TSA+DETA~[3] & ICCV2023 & ResNet18 & Metric & & \cmark & \cmark & 51.42 & 61.58 \\ 
            PUTM~[4] & ICCV2023 & ResNet18 & Metric & & \cmark & \cmark & 60.23 & 72.36 \\
            FRN~[5] & CVPR2021
            & ResNet12 & Fine-tuning  & \cmark & & \cmark & 50.23 & 60.56  \\
            Yang et al~[6] & ECCV2022 & ResNet12 & Fine-tuning  & \cmark & & \cmark & 58.01 & 69.32 \\
            LP-FT-FB~[7] & ICLR2023
            & ResNet12 & Fine-tuning & \cmark & \cmark & \cmark & 56.21  & 70.21 \\ 
            \shline
    \end{tabular}
} 
\label{tab:fsc_acc}
\end{table}

\begin{table}[htbp]  
    \centering
    \caption{Experiments in few-shot classification by using vision-language pre-trained models. Two vision backbones following their original paper are considered, \textit{i.e.}, ResNet50 and ViT-B/16.}
    \vspace{-3mm}
    % \scalebox{0.86}{
    \resizebox{1.0\textwidth}{!}{
        \begin{tabular}{lccc|ccc|ccc}
            \shline
            & & & & \multicolumn{3}{c|}{$1$-shot} & \multicolumn{3}{c}{$16$-shot} \\
            Method & Conference & Backbone & Type & Base & New & HM 
            & Base & New & HM \\
            \hline
            CLIP~[8] & CVPR2021 & ResNet50 & Zero-shot CLIP & 68.12 & 72.19 & 70.10 & 68.12 & 72.19 & 70.10   \\
            CoOp~[9] & ICLR2022 & ResNet50 & Prompt-tuning CLIP & 61.22 & 63.62 & 62.40 & 47.55 & 40.90 & 43.98  \\ 
            CoCoOp~[10] & CVPR2022 & ResNet50 & Prompt-tuning CLIP & 59.86 & 63.88 & 61.80 & 36.88 & 46.10 & 40.98 \\
            KgCoOp~[11] & CVPR2023 & ResNet50 & Prompt-tuning CLIP & 67.95 & 72.05 & 69.94 & 49.18 & 48.78 & 48.98 \\
            LFA~[13] & ICCV2023 & ResNet50 & Prompt-tuning CLIP & 66.87 & 73.01 & 69.81 & 49.23 & 48.12 & 48.67 \\
            ProGrad~[14] & ICCV2023 & ResNet50 & Prompt-tuning CLIP & 65.23 & 69.39 & 67.25 & 49.14 & 47.36 & 48.23 \\
            \hline \hline
            CLIP~[8] & CVPR2021 & ViT-B/16 & Zero-shot CLIP & 73.19 & 75.29 & 74.23 & 73.19 & 75.29 & 74.23  \\
            CoOp~[9] & ICLR2022 & ViT-B/16 & Prompt-tuning CLIP & 64.95 & 68.87 & 66.85 &  49.98 & 45.40 & 47.58  \\ 
            CoCoOp~[10] & CVPR2022 & ViT-B/16 & Prompt-tuning CLIP & 65.60 & 69.50 & 67.49 & 49.35 & 47.84 & 48.58 \\
            KgCoOp~[11] & CVPR2023 & ViT-B/16 & Prompt-tuning CLIP & 71.22 & 74.74 & 72.94 & 51.21 & 50.99 & 51.10 \\
            MaPLe~[12] & CVPR2023 & ViT-B/16 & Prompt-tuning CLIP & 60.31 & 68.94 & 64.34 & 48.04 & 49.47 &  48.74 \\
            LFA~[13] & ICCV2023 & ViT-B/16 & Prompt-tuning CLIP & 71.56 & 74.98 & 73.23 & 52.04 & 49.65 & 50.82 \\
            ProGrad~[14] & ICCV2023 & ViT-B/16 & Prompt-tuning CLIP & 70.81 & 73.27 & 72.02 & 51.48 & 48.02 & 49.69 \\
            \shline
    \end{tabular}
} 
\label{tab:fsc_acc}
\end{table}

\textbf{Reference}

[1] Tianjun Ke et al. Revisiting Logistic-softmax Likelihood in Bayesian Meta-learning for Few-shot Classification. NeurIPS2023.

[2] Jiangtao Xie et al. Joint Distribution Matters: Deep Brownian Distance Covariance for Few-Shot Classification. CVPR2022.

[3] Ji Zhang et al. DETA: Denoised Task Adaptation for Few-Shot Learning. ICCV2023. 

[4] Long Tian et al. Prototypes-oriented Transductive Few-shot Learning with Conditional Transport. ICCV2023.

[5] Wertheimer Davis et al. Few-shot classification with feature map reconstruction networks. CVPR2021. 

[6] Zhanyuan Yang et al. Few-shot classification with contrastive learning. ECCV2022. 

[7] Heng Wang et al. Revisit Finetuning strategy for Few-Shot Learning to Transfer the Emdeddings. ICLR2023.

[8] Radford Alec et al. Learning transferable visual models from natural language supervision. ICML2021.

[9] Kaiyang Zhou et al. Learning to prompt for vision-language models. IJCV2022.

[10] Kaiyang Zhou et al. Conditional prompt learning for vision-language models. CVPR2022.

[11] Haotao Yao et al. Visual-Language Prompt Tuning with Knowledge-guided Context Optimization. CVPR2023.

[12] Muhammad Uzair Khattak et al. MaPLe: Multi-modal Prompt Learning. CVPR2023.

[13] Yassine Ouali et al. Black Box Few-Shot Adaptation for Vision-Language models. ICCV2023.

[14] Beier Zhu et al. Prompt-aligned Gradient for Prompt Tuning. ICCV2023.

\textbf{How to understand the conceptual and contextual information mentioned in the manuscript?}


\textbf{More explanations about the network structure ResNet50.}

We apologize for the missing explanation for ResNet50. The network structure of ResNet50 is same as the existing works [1,2] and is pre-trained using the self-supervised loss. Specifically, it contains four blocks and each block has 3-layer bottleneck block. 

\textbf{Reference}

[1] Kaiming He et al. Momentum Contrast for Unsupervised Visual Representation Learning. CVPR2020.

[2] Ting Chen et al. A Simple Framework for Contrastive Learning of Visual Representations. ICML2020.




==> tables/data.tex <==
\begin{table}
\centering
\renewcommand{\arraystretch}{1.2}
\renewcommand{\tabcolsep}{1.2mm}
\resizebox{\linewidth}{!}{
\begin{tabular}{|l l l l l l l l l l l l l l l l l l l l l l l l|}
\hline
\cline{1-24}
              \multicolumn{24}{|c|}{\textcolor{blue}{Animal}}\\
\cline{1-24}
\hline
\textbf{class} & dog & cat & bird & bear & horse & cow & elephant & sheep & monkey & lion & squirrel & wolf & lizard & tiger & giraffe & owl & seal & frog & rabbit & goose &  kangaroo & fox & butterfly \\
\hline
\textbf{total} &  & 135 & 45 & 500 & 517 & 210 & 1507 & \\
grass & 197 & 180 & 46 & 500 & 724 & 188 & 1835 & \\
water & 71 & 47 & 167 & 500 & 662 & 290 & 1737 \\
outdoor & 35 & 63 & 38 & 500 & 217 & 25 & 878 & \\
dim & 94 & 148 & 53 & 500 & 320 & 96 & 1211 & \\
white & 0 & 0 & 0 & 500 & 517 & 210 & 1507 & \\
rock & 197 & 180 & 46 & 500 & 724 & 188 & 1835 & \\
autumn & 71 & 47 & 167 & 500 & 662 & 290 & 1737  \\
black & 35 & 63 & 38 & 500 & 217 & 25 & 878 & \\
brown \\
wood \\
blue \\
green \\
gray \\
on snow \\
large \\
eating \\
red \\
metal \\
lying \\
with people \\
on beach \\
small \\
in forest \\
on road \\
silver \\
running \\
in cage \\
open \\
yellow \\
standing \\
in city \\
sitting \\
tall \\
in river \\
in water \\
dark \\
at home \\
walking \\
glass \\
orange \\
on tree \\
in hand \\
flying \\
plastic \\
long \\
closed \\
on ground \\
aside mountain \\
pink \\
round \\
bare \\
tan \\
baby \\
in garage \\
yacht \\
on track \\
at station \\
wooden \\
in farm \\
on branch \\
leafy \\
shared \\
velodrome \\
at wharf \\
double decker \\
on \\
cross bridge \\
in sunset \\
at heliport \\
on bridge \\
in burrow \\
aside tree \\
in zoo \\
in pot \\
at airport \\
on sea \\
sleeping \\
in desert \\
eating grass \\
in race \\
taking off \\
on power line \\
in circus \\
mountain \\
short \\
\hline
\end{tabular}
}
\caption{Detailed statistics of the dataset.}
\label{dataset_1}
\end{table}


\begin{table}
\centering
\renewcommand{\arraystretch}{1.2}
\renewcommand{\tabcolsep}{1.2mm}
\resizebox{\linewidth}{!}{
\begin{tabular}{|l l l l l l l l l l l l l l l l l l l l l l l l|}
\hline
\cline{1-24}
              \multicolumn{24}{|c|}{\textcolor{blue}{Animal}}\\
\cline{1-24}
\hline
\textbf{class} & dog & cat & bird & bear & horse & cow & elephant & sheep & monkey & lion & squirrel & wolf & lizard & tiger & giraffe & owl & seal & frog & rabbit & goose &  kangaroo & fox & butterfly \\
\hline
\textbf{total} &  & 135 & 45 & 500 & 517 & 210 & 1507 & \\
open mouth \\
on booth \\
howling \\
brick \\
khaki \\
at dock \\
on head \\
around cloud \\
climbing \\
stone \\
on web \\
on a stick \\
leather \\
cutting \\
concrete \\
at park \\
on iceberg \\
on shoulder \\
at night \\
with flower \\
grazing \\
paper \\
spotted \\
at yard \\
with bee \\
hanging \\
clean \\
square \\
subway \\
jumping \\
on flower \\
landing \\
porcelain \\
at sunset \\
on desk \\
fighting \\
purple \\
off \\
gold \\
dirty \\
resting \\
beige \\
rectangular \\
thin \\
thick \\
in bucket \\
city \\
in pouch \\
in hole \\
on bird feeder \\
on shelves \\
on wall \\
on post \\
in box \\
shiny \\
sinking \\
with cargo \\
bright \\
in shell \\
aside traffic light \\
empty \\
cross tunnel \\
full \\
playing \\
light brown \\
staring \\
colorful \\
dark brown \\
young \\
dark blue \\
\hline
\end{tabular}
}
\caption{Detailed statistics of the dataset.}
\label{dataset_2}
\end{table}


==> tables/iid_ood_episode_acc.tex <==
\begin{table}[tbp]  
    \centering
    % \scalebox{0.86}{
    \resizebox{1.0\textwidth}{!}{
        \begin{tabular}{lc|cc|cc}
            \shline
            Method & Type & $5$-w $1$-s (OOD) & $5$-w $5$-s (OOD) & $5$-w $1$-s (IID) & $5$-w $5$-s (IID) \\ 
            \hline 
            \textbf{CAN}~\citep{hou2019cross}  & Metric  & 48.69 \scriptsize$\pm$ 0.47 & 61.04 \scriptsize$\pm$ 0.44 & 49.50 \scriptsize$\pm$ 0.47 & 62.43 \scriptsize$\pm$ 0.43 \\
            \textbf{ProtoNet}~\citep{snell2017prototypical}  & Metric  & 41.85 \scriptsize$\pm$ 0.41 & 57.26 \scriptsize$\pm$ 0.42 & 43.06 \scriptsize$\pm$ 0.41 & 59.14 \scriptsize$\pm$ 0.43 \\
            \textbf{Versa}~\citep{gordon2018versa}  & Meta  & 39.67 \scriptsize$\pm$ 0.40 & 52.75 \scriptsize$\pm$ 0.41 & 40.10 \scriptsize$\pm$ 0.39 & 54.00 \scriptsize$\pm$ 0.42 \\
            \textbf{ANIL}~\citep{RaghuRBV20}  & Meta  & 36.54 \scriptsize$\pm$ 0.40 & 49.15 \scriptsize$\pm$ 0.42 & 37.79 \scriptsize$\pm$ 0.41 & 50.77 \scriptsize$\pm$ 0.43 \\
            \textbf{R2D2}~\citep{bertinetto2018meta}  & Meta  & 43.48 \scriptsize$\pm$ 0.42 & 58.21 \scriptsize$\pm$ 0.41 & 44.71 \scriptsize$\pm$ 0.42 & 59.89 \scriptsize$\pm$ 0.42 \\
            \textbf{DN4}~\citep{li2019revisiting}  & Metric  & 44.44 \scriptsize$\pm$ 0.42 & 56.03 \scriptsize$\pm$ 0.42 & 45.61 \scriptsize$\pm$ 0.43 & 58.18 \scriptsize$\pm$ 0.43\\
            \textbf{Baseline}~\citep{ChenLKWH19}  & Fine-tuning  & 44.01 \scriptsize$\pm$ 0.40 & 57.22 \scriptsize$\pm$ 0.41 & 45.54 \scriptsize$\pm$ 0.41 & 59.51 \scriptsize$\pm$ 0.40 \\
            \textbf{Baseline++}~\citep{ChenLKWH19}  & Fine-tuning  & 44.97 \scriptsize$\pm$ 0.43 & 57.01 \scriptsize$\pm$ 0.41 & 46.37 \scriptsize$\pm$  0.45 &  58.14 \scriptsize$\pm$ 0.41 \\
            \shline
        \end{tabular}
    } 
\caption{different and same context 5 way}
\label{tab:iid_ood_acc}
\end{table}

==> tables/single_methods.tex <==
\begin{table}[tbp]  
    \centering
    % \scalebox{0.66}{
    \resizebox{1.0\textwidth}{!}{
        \begin{tabular}{lrcccccccc|cc|cc}
            \shline
            Method & Backbone & Type & Parameter & PT & GL & LL & TT & SS & DA & $5$-w $1$-s & $5$-w $5$-s & $5$-w $1$-s (iid) & $5$-w $5$-s (iid) \\ 
            \hline
            \textbf{Baseline}~\citep{ChenLKWH19}          
            & Conv64F & Fine-tuning & $0.22$M 
            & & \cmark & & \cmark & & & 37.97 & 52.08   \\
            \textbf{Baseline++}~\citep{ChenLKWH19}            
            & Conv64F & Fine-tuning & $0.22$M   
            & & \cmark & & \cmark & & & 40.45 & 53.42  \\
            \textbf{RFS-simple}~\citep{tian2020rethinking}        
            & Conv64F & Fine-tuning  & $0.22$M 
            & & & & &  &         \\
            \textbf{Neg-Cosine}~\citep{liu2020negative} 
            & Conv64F & Fine-tuning  & $0.22$M 
            & & &  &   &    &        \\
            \textbf{SKD-GEN0}~\citep{rajasegaran2020self}  
            & Conv64F   & Fine-tuning  & $0.22$M  
            & & &  &  &  &      \\
            \hdashline[1pt/1pt]
            \textbf{MAML}~\citep{FinnAL17}            
            & Conv64F & Meta  & $0.12$M  
            &  &  & \cmark & \cmark & & &   &         \\
            \textbf{Versa}~\citep{gordon2018versa}       
            & Conv64F  & Meta  & $1.18$M     
            &   &   &   &&& & 20.00 & 51.95        \\
            \textbf{R2D2}~\citep{bertinetto2018meta}   
            & Conv64F   & Meta  & $0.11$M     
            &   &  & & & & & 39.56 &  51.29       \\
            \textbf{MTL}~\citep{sun2019meta}     
            & Conv64F & Meta  & $1.80$M  
            & \cmark & \cmark & \cmark & \cmark & &          \\
            \textbf{ANIL}~\citep{RaghuRBV20}        
            & Conv64F & Meta  & $0.12$M      
            & & & \cmark & \cmark & & & 37.24 & 48.04              \\
            \textbf{BOIL}~\citep{oh2020boil}    
            & Conv64F & Meta & $0.12$M 
            &  & & \cmark & \cmark & & &  &        \\
            \hdashline[1pt/1pt]
            \textbf{ProtoNet}~\citep{snell2017prototypical}  
            & Conv64F  & Metric   & $0.11$M   
            &  & & \cmark & & & & 37.92 & 51.39            \\
            \textbf{RelationNet}~\citep{sung2017learning}    
            & Conv64F & Metric & $0.23$M   
            &  &  & \cmark & & &  &         \\
            \textbf{CovaMNet}~\citep{li2019distribution} 
            & Conv64F    & Metric  & $0.11$M      
            &  &    &     &&&    &         \\
            \textbf{DN4}~\citep{li2019revisiting} 
            & Conv64F    & Metric  & $0.11$M 
            &  &  & \cmark & & & & 38.87 & 52.72           \\
            \textbf{CAN}~\citep{hou2019cross}         
            & Conv64F  & Metric & $0.13$M      
            & \cmark & \cmark & \cmark & && & 43.02 &  55.48             \\
            \textbf{RENet}~\citep{kang2021relational}     
            & Conv64F  & Metric  & $0.20$M      
            &    & & &   &   &      \\
            \hline\hline
            \textbf{Baseline}~\citep{ChenLKWH19}      
            & ResNet12  & Fine-tuning  & $12.47$M    
            & & \cmark & & \cmark & & & 46.78   & 60.78    & 91.18/69.57 & 91.11/87.46    \\
            \textbf{Baseline++}~\citep{ChenLKWH19}  
            & ResNet12     & Fine-tuning  &  $12.47$M  & & \cmark & & \cmark & &  & 46.95 & 58.50  & 90.93/84.94 & 91.03/93.68      \\
            \textbf{RFS-simple}~\citep{tian2020rethinking} 
            & ResNet12     & Fine-tuning  &  $12.47$M    &   &   &&&   &       &         \\
            \textbf{Neg-Cosine}~\citep{liu2020negative} 
            & ResNet12     & Fine-tuning  &  $12.47$M    &   &  &&&    &        &          \\
            \textbf{SKD-GEN0}~\citep{rajasegaran2020self}  
            & ResNet12     & Fine-tuning  &  $12.47$M    &   &  &&&    &    &      \\
            \hdashline[1pt/1pt]
            \textbf{MAML}~\citep{FinnAL17}                
            & ResNet12  & Meta         
            &  &  & \cmark & \cmark & & &    &    \\
            \textbf{Versa}~\citep{gordon2018versa}  
            & ResNet12     & Meta         &  $13.25$M    & &     &&&  &  &    39.64 & 53.06 & 54.69/56.66 & 78.49/78.15           \\
            \textbf{R2D2}~\citep{bertinetto2018meta}   
            & ResNet12     & Meta         &  $12.42$M    &  &   &&&   &  &   45.25 & 60.14  & 80.81/83.45 & 95.44/94.82            \\
            \textbf{MTL}~\citep{sun2019meta}      
            & ResNet12     & Meta         & $13.13$M  & \cmark & \cmark & \cmark & \cmark &    &      \\
            \textbf{ANIL}~\citep{RaghuRBV20}     
            & ResNet12     & Meta         &  $12.43$M    &  &    &&&  &  &  36.58 & 50.54    & 67.58/63.77   & 87.59/90.42       \\
            \textbf{BOIL}~\citep{oh2020boil}     
            & ResNet12     & Meta         &  $12.43$M    &  &  &&&      &         &          \\
            \hdashline[1pt/1pt]
            \textbf{ProtoNet}~\citep{snell2017prototypical}  
            & ResNet12   & Metric  & $12.42$M  &  & & \cmark & & & & 42.69 & 59.50 & 63.24/67.07 & 92.75/93.70            \\
            \textbf{RelationNet}~\citep{sung2017learning}     
            & ResNet12     & Metric       &  $23.53$M    &   & &       &&&          &       &        \\
            \textbf{CovaMNet}~\citep{li2019distribution}     
            & ResNet12     & Metric       &  $12.42$M    &   & &       &&&          &         &       \\
            \textbf{DN4}~\citep{li2019revisiting}        
            & ResNet12     & Metric       &  $12.42$M    &   & &       &&&          &   45.04 & 57.68 & 82.67/82.49 & 93.45/92.88            \\
            \textbf{CAN}~\citep{hou2019cross}          
            & ResNet12     & Metric       &  $12.65$M    & & &  &&&      &   48.93 & 62.36 & 92.90/93.11 & 96.30/96.68             \\
            \textbf{RENet}~\citep{kang2021relational}      
            & ResNet12     & Metric       &  $12.67$M    &&       &&&   &    &     \\
            \hline\hline
            \textbf{Baseline}~\citep{ChenLKWH19}       
            & ResNet18     & Fine-tuning  & $11.20$M & & \cmark & & \cmark & & & 46.49 & 60.22        \\
            \textbf{Baseline++}~\citep{ChenLKWH19}   
            & ResNet18     & Fine-tuning  & $11.20$M & & \cmark & & \cmark & & & 47.26 & 60.10       \\
            \textbf{RFS-simple}~\citep{tian2020rethinking} 
            & ResNet18     & Fine-tuning  & $11.20$M     &    &  &&    &    &       \\
            \textbf{Neg-Cosine}~\citep{liu2020negative} 
            & ResNet18     & Fine-tuning &$11.20$M      &     & &&&   &        &           \\
            \textbf{SKD-GEN0}~\citep{rajasegaran2020self} 
            & ResNet18     & Fine-tuning & $11.20$M     &     &   &&& &    &    \\
            \hdashline[1pt/1pt]
            \textbf{MAML}~\citep{FinnAL17}                
            & ResNet18  & Meta         
            &  &  & \cmark & \cmark & & &  &    \\
            \textbf{Versa}~\citep{gordon2018versa}    
            & ResNet18      & Meta         &  $11.96$M    & &  &   &&&    &  38.88 & 53.18              \\
            \textbf{R2D2}~\citep{bertinetto2018meta}   
            & ResNet18      & Meta         &  $11.17$M    & &  &   &&&    &  45.26 & 58.53               \\
            \textbf{MTL}~\citep{sun2019meta}           
            & ResNet18   & Meta   & $11.88$M & \cmark & \cmark & \cmark & \cmark   &  &      \\
            \textbf{ANIL}~\citep{RaghuRBV20}       
            &ResNet18      & Meta         &  $11.17$M    &  && &&&    &       37.26 & 49.42         \\
            \textbf{BOIL}~\citep{oh2020boil}   
            & ResNet18      & Meta         &  $11.17$M    &  &&     &     &&&    &          \\
            \hdashline[1pt/1pt]
            \textbf{ProtoNet}~\citep{snell2017prototypical}  
            & ResNet18  & Metric  & $11.17$M  &  & & \cmark & & & & 43.14 & 57.84    \\
            \textbf{RelationNet}~\citep{sung2017learning} 
            & ResNet18      & Metric       &  $18.29$M    &   &       &      &&&     &      &       \\
            \textbf{CovaMNet}~\citep{li2019distribution}   & \textit{ResNet18}      & Metric       &  $11.16$M    & - & - & - & - & - \\
            \textbf{DN4}~\citep{li2019revisiting}      
            & ResNet18      & Metric       &  $11.17$M    &   &\cmark      &      &&&         &    43.73  &  56.56           \\
            \textbf{CAN}~\citep{hou2019cross}            
            & ResNet18      & Metric       &  $11.35$M    & &   &&&&     &       48.18 & 62.38      \\
            \textbf{RENet}~\citep{kang2021relational} 
            & ResNet18      & Metric       & $11.52$M     & &   &&&     &    \\
            \shline
    \end{tabular}} 
\caption{\textbf{The overview picture of the state of the art} on \textit{mini}ImageNet and \textit{tiered}ImageNet by controlling the most common implementation details except some special tricks, with our \textbf{LibFewShot}. The fifth column shows the total number of trainable parameters used by each method. Global-label indicates that the global labels of the auxiliary set are used for pre-training or global classification during training. Local-label means that only the specific local labels are used in the episodic- or meta-training phase. Test-tune means test-tuning of using the support set at the test stage. Note that SKD-GEN0 uses an additional self-supervision trick that is the core of this method.}
\label{Table2_SOTA}
\end{table}

==> tables/singler_methods.tex <==
\begin{table*}[tbp]  
    \centering
    % \scalebox{0.6}{
    \resizebox{1.0\textwidth}{!}{
        \begin{tabular}{lrccccc|cc}
            \shline
            Method & Backbone & Type & Parameter & Global-label &Local-label & Test-tune & $5$-way $1$-shot & $5$-way $5$-shot \\ 
            \hline
            \textbf{Baseline}~\citep{ChenLKWH19}          
            & Conv64F & Non-episodic & $0.22$M 
            & \cmark & & \cmark  & 37.97 \footnotesize$\pm$ 0.32 & 52.08 \footnotesize$\pm$ 0.35   \\
            \textbf{Baseline++}~\citep{ChenLKWH19}            
            & Conv64F & Non-episodic & $0.22$M   
            & \cmark & & \cmark  & 40.45 \footnotesize$\pm$ 0.36 & 53.42 \footnotesize$\pm$ 0.37       \\
            \textbf{RFS-simple}~\citep{TianWKTI20_RFS}        
            & Conv64F & Non-episodic  & $0.22$M 
            & \cmark & & \cmark &  &         \\
            \textbf{Neg-Cosine}~\citep{Negative-cosine_ECCV20} 
            & Conv64F & Non-episodic  & $0.22$M 
            & \cmark & & \cmark &    &        \\
            \textbf{SKD-GEN0}~\citep{rajasegaran2020self_SKD}  
            & Conv64F   & Non-episodic  & $0.22$M  
            & \cmark & & \cmark &   &      \\
            \hdashline[1pt/1pt]
            \textbf{MAML}~\citep{finn2017model}            
            & Conv64F & Meta  & $0.12$M  
            &   & \cmark  & \cmark  &       &         \\
            \textbf{Versa}~\citep{gordon2018versa}       
            & Conv64F  & Meta  & $1.18$M     
            &   & \cmark  & \cmark  & 20.00 \footnotesize$\pm$ 0.00  & 51.95 \footnotesize$\pm$ 0.35         \\
            \textbf{R2D2}~\citep{BertinettoHTV19_R2D2}   
            & Conv64F   & Meta  & $0.11$M     
            &   & \cmark  & \cmark  & 39.56 \footnotesize$\pm$ 0.36 &  51.29 \footnotesize$\pm$ 0.36       \\
            \textbf{LEO}~\citep{RusuRSVPOH19_LEO}  
            & Conv64F  & Meta   & $1.20$M      
            & \cmark & \cmark & \cmark &  &    \\
            \textbf{MTL}~\citep{sun2019meta}     
            & Conv64F & Meta  & $1.80$M  
            & \cmark & \cmark & \cmark &   &          \\
            \textbf{ANIL}~\citep{raghu2020ANIL}        
            & Conv64F & Meta  & $0.12$M      
            &  & \cmark & \cmark  & 37.24 \footnotesize$\pm$ 0.36 & 48.04 \footnotesize$\pm$ 0.39              \\
            \textbf{BOIL}~\citep{OhYKY2021BOIL}    
            & Conv64F & Meta & $0.12$M 
            &  & \cmark & \cmark &      &        \\
            \hdashline[1pt/1pt]
            \textbf{ProtoNet}~\citep{snell2017prototypical}  
            & Conv64F  & Metric    & $0.11$M   
            &  & \cmark &  &  37.92 \footnotesize$\pm$ 0.35 & 51.39 \footnotesize$\pm$ 0.38            \\
            \textbf{RelationNet}~\citep{sung2018learning}    
            & Conv64F & Metric & $0.23$M   
            &  & \cmark &   &   &         \\
            \textbf{CovaMNet}~\citep{li2019distribution} 
            & Conv64F    & Metric  & $0.11$M      
            &  & \cmark &    &        &         \\
            \textbf{DN4}~\citep{li2019revisiting} 
            & Conv64F    & Metric  & $0.11$M 
            &  & \cmark &  &    38.87 \footnotesize$\pm$ 0.36 & 52.72 \footnotesize$\pm$ 0.38           \\
            \textbf{CAN}~\citep{hou2019cross}         
            & Conv64F  & Metric & $0.13$M      
            & \cmark  & \cmark  &   & 43.02 \footnotesize$\pm$ 0.42 &  55.48 \footnotesize$\pm$ 0.40             \\
            \textbf{RENet}~\citep{kang2021renet}     
            & Conv64F  & Metric  & $0.20$M      
            & \cmark & \cmark  &     &   &      \\
            \hline\hline
            \textbf{Baseline}~\citep{ChenLKWH19}      
            & ResNet12  & Non-episodic  & $12.47$M    
            & \cmark &  & \cmark   & 46.78 \footnotesize$\pm$ 0.41   & 60.78 \footnotesize$\pm$ 0.40        \\
            \textbf{Baseline++}~\citep{ChenLKWH19}  
            & ResNet12     & Non-episodic  &  $12.47$M    &  \cmark &  &  \cmark      &  46.95 \footnotesize$\pm$ 0.42     & 58.50 \footnotesize$\pm$ 0.36        \\
            \textbf{RFS-simple}~\citep{TianWKTI20_RFS} 
            & ResNet12     & Non-episodic  &  $12.47$M    &  \cmark &  &  \cmark      &       &         \\
            \textbf{Neg-Cosine}~\citep{Negative-cosine_ECCV20} 
            & ResNet12     & Non-episodic  &  $12.47$M    &  \cmark &  &  \cmark      &        &          \\
            \textbf{SKD-GEN0}~\citep{rajasegaran2020self_SKD}  
            & ResNet12     & Non-episodic  &  $12.47$M    &  \cmark &  &  \cmark      &    &      \\
            \hdashline[1pt/1pt]
            \textbf{MAML}~\citep{finn2017model}                
            & ResNet12  & Meta         
            & -  & -  & -   & -   & -   & -   \\
            \textbf{Versa}~\citep{gordon2018versa}  
            & ResNet12     & Meta         &  $13.25$M    & &\cmark  &  \cmark         &    39.64 \footnotesize$\pm$ 0.39 & 53.06 \footnotesize$\pm$ 0.40              \\
            \textbf{R2D2}~\citep{BertinettoHTV19_R2D2}   
            & ResNet12     & Meta         &  $12.42$M    &  &\cmark &  \cmark         &   45.25 \footnotesize$\pm$ 0.42 & 60.14 \footnotesize$\pm$ 0.37              \\
            \textbf{LEO}~\citep{RusuRSVPOH19_LEO}     
            & ResNet12     & Meta         &  $12.60$M    &\cmark &\cmark &\cmark  &        &       \\
            \textbf{MTL}~\citep{sun2019meta}      
            & ResNet12     & Meta         & $13.13$M     &\cmark &\cmark &\cmark  &    &      \\
            \textbf{ANIL}~\citep{raghu2020ANIL}     
            & ResNet12     & Meta         &  $12.43$M    &  &\cmark  &\cmark          &  36.58 \footnotesize$\pm$ 0.38 & 50.54 \footnotesize$\pm$ 0.40             \\
            \textbf{BOIL}~\citep{OhYKY2021BOIL}     
            & ResNet12     & Meta         &  $12.43$M    &  &\cmark  & \cmark         &         &          \\
            \hdashline[1pt/1pt]
            \textbf{ProtoNet}~\citep{snell2017prototypical}  
            & ResNet12     & Metric       &  $12.42$M    &   &\cmark    &                &   42.69 \footnotesize$\pm$ 0.39 & 59.50 \footnotesize$\pm$ 0.40              \\
            \textbf{RelationNet}~\citep{sung2018learning}     
            & ResNet12     & Metric       &  $23.53$M    &   &\cmark    &                &       &        \\
            \textbf{CovaMNet}~\citep{li2019distribution}     
            & ResNet12     & Metric       &  $12.42$M    &   &\cmark    &                &         &       \\
            \textbf{DN4}~\citep{li2019revisiting}        
            & ResNet12     & Metric       &  $12.42$M    &   &\cmark    &                &   45.04 \footnotesize$\pm$ 0.39 & 57.68 \footnotesize$\pm$ 0.39             \\
            \textbf{CAN}~\citep{hou2019cross}          
            & ResNet12     & Metric       &  $12.65$    &\cmark &\cmark    &        &   48.93 \footnotesize$\pm$ 0.42 & 62.36 \footnotesize$\pm$ 0.40              \\
            \textbf{RENet}~\citep{kang2021renet}      
            & ResNet12     & Metric       &  $12.67$M    &\cmark &\cmark   &         &    &     \\
            \hline\hline
            \textbf{Baseline}~\citep{ChenLKWH19}       
            & ResNet18     & Non-episodic  & $11.20$M     &  \cmark  &  &  \cmark     & 46.49 \footnotesize$\pm$ 0.41        & 60.22 \footnotesize$\pm$ 0.39         \\
            \textbf{Baseline++}~\citep{ChenLKWH19}   
            & ResNet18     & Non-episodic  & $11.20$M     &  \cmark  & &  \cmark      & 47.26 \footnotesize$\pm$ 0.40       &  60.10 \footnotesize$\pm$ 0.38        \\
            \textbf{RFS-simple}~\citep{TianWKTI20_RFS} 
            & ResNet18     & Non-episodic  & $11.20$M     &  \cmark  &  &  \cmark     &    &       \\
            \textbf{Neg-Cosine}~\citep{Negative-cosine_ECCV20} 
            & ResNet18     & Non-episodic  &$11.20$M      &  \cmark  &   & \cmark     &        &           \\
            \textbf{SKD-GEN0}~\citep{rajasegaran2020self_SKD} 
            & ResNet18     & Non-episodic  & $11.20$M     &  \cmark  &   &  \cmark    &    &    \\
            \hdashline[1pt/1pt]
            \textbf{MAML}~\citep{finn2017model}                
            & ResNet18  & Meta         
            & -  & -  & -   & -   & -   & -   \\
            \textbf{Versa}~\citep{gordon2018versa}    
            & ResNet18      & Meta         &  $11.96$M    & &\cmark &\cmark           &  38.88 \footnotesize$\pm$ 0.36 & 53.18 \footnotesize$\pm$ 0.36              \\
            \textbf{R2D2}~\citep{BertinettoHTV19_R2D2}   
            & ResNet18      & Meta         &  $11.17$M    & &\cmark &\cmark           &  45.26 \footnotesize$\pm$ 0.38 & 58.53 \footnotesize$\pm$ 0.38               \\
            \textbf{LEO}~\citep{RusuRSVPOH19_LEO}      
            & ResNet18      & Meta         &  $11.31$M    &\cmark &\cmark &\cmark &         &        \\
            \textbf{MTL}~\citep{sun2019meta}           
            & ResNet18      & Meta         &  $11.88$M    &\cmark &\cmark &\cmark &   &      \\
            \textbf{ANIL}~\citep{raghu2020ANIL}       
            &ResNet18      & Meta         &  $11.17$M    &  &\cmark   &\cmark        &       37.26 \footnotesize$\pm$ 0.36 & 49.42 \footnotesize$\pm$ 0.39          \\
            \textbf{BOIL}~\citep{OhYKY2021BOIL}   
            & ResNet18      & Meta         &  $11.17$M    &  &\cmark   & \cmark       &        &          \\
            \hdashline[1pt/1pt]
            \textbf{ProtoNet}~\citep{snell2017prototypical}  
            & ResNet18      & Metric       &  $11.17$M    &  &\checkmark  &  &  43.14 \footnotesize$\pm$ 0.37 & 57.84 \footnotesize$\pm$ 0.39           \\
            \textbf{RelationNet}~\citep{sung2018learning} 
            & ResNet18      & Metric       &  $18.29$M    &   &\checkmark          &          &      &       \\
            \textbf{CovaMNet}~\citep{li2019distribution}   & \textit{ResNet18}      & Metric       &  $11.16$M    & - & - & - & - & - \\
            \textbf{DN4}~\citep{li2019revisiting}      
            & ResNet18      & Metric       &  $11.17$M    &   &\checkmark      &              &    43.73 \footnotesize$\pm$ 0.38  &  56.56 \footnotesize$\pm$ 0.39           \\
            \textbf{CAN}~\citep{hou2019cross}            
            & ResNet18      & Metric       &  $11.35$M    &\cmark & \cmark    &       &       48.18 \footnotesize$\pm$ 0.42 & 62.38 \footnotesize$\pm$ 0.41      \\
            \textbf{RENet}~\citep{kang2021renet} 
            & ResNet18      & Metric       & $11.52$M     &\cmark &  \cmark   &       &    \\
            \shline
    \end{tabular}} 
\caption{\textbf{The overview picture of the state of the art} on \textit{mini}ImageNet and \textit{tiered}ImageNet by controlling the most common implementation details except some special tricks, with our \textbf{LibFewShot}. The fifth column shows the total number of trainable parameters used by each method. Global-label indicates that the global labels of the auxiliary set are used for pre-training or global classification during training. Local-label means that only the specific local labels are used in the episodic- or meta-training phase. Test-tune means test-tuning of using the support set at the test stage. Note that SKD-GEN0 uses an additional self-supervision trick that is the core of this method.}
\label{Table2_SOTA}
\end{table*}
